DEXTER: An end-to-end system to extract table contents from electronic medical health documents

In this paper, we propose DEXTER, an end to end system to extract information from tables present in medical health documents, such as electronic health records (EHR) and explanation of benefits (EOB). DEXTER consists of four sub-system stages: i) table detection ii) table type classification iii) cell detection; and iv) cell content extraction. We propose a two-stage transfer learning-based approach using CDeC-Net architecture along with Non-Maximal suppression for table detection. We design a conventional computer vision-based approach for table type classification and cell detection using parameterized kernels based on image size for detecting rows and columns. Finally, we extract the text from the detected cells using pre-existing OCR engine Tessaract. To evaluate our system, we manually annotated a sample of the real-world medical dataset (referred to as Meddata) consisting of wide variations of documents (in terms of appearance) covering different table structures, such as bordered, partially bordered, borderless, or coloured tables. We experimentally show that DEXTER outperforms the commercially available Amazon Textract and Microsoft Azure Form Recognizer systems on the annotated real-world medical dataset

==> old_tables.tex <==
% Scores for bordered table detection BUDDI vs amazon
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{IoU} & \multicolumn{4}{c|}{BUDDI Dexter}   & \multicolumn{4}{c|}{AMAZON Textract} \\ \cline{2-9} 
                     & Precision & Recall & F1   & mAP     & Precision  & Recall & F1   & mAP     \\ \hline
0.5                  & 0.94      & 0.97   & 0.95 & 96.80\% & 0.96       & 0.78   & 0.86 & 77.68\% \\ \hline
0.6                  & 0.94      & 0.97   & 0.95 & 96.80\% & 0.96       & 0.78   & 0.86 & 77.68\% \\ \hline
0.7                  & 0.92      & 0.95   & 0.94 & 95.03\% & 0.9        & 0.73   & 0.81 & 72.58\% \\ \hline
0.8                  & 0.86      & 0.89   & 0.88 & 87.76\% & 0.9        & 0.73   & 0.81 & 72.58\% \\ \hline
0.9                  & 0.58      & 0.6    & 0.59 & 56.98\% & 0.82       & 0.67   & 0.74 & 63.19\% \\ \hline
\end{tabular}
\caption{Table Detection scores on the bordered split of the custom dataset}
\label{tab:table_detection_bordered_split}
\end{table}

% Scores for borderless table detection BUDDI vs amazon
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{IoU} & \multicolumn{4}{c|}{BUDDI Dexter}   & \multicolumn{4}{c|}{AMAZON Textract} \\ \cline{2-9} 
                     & Precision & Recall & F1   & mAP     & Precision  & Recall & F1   & mAP     \\ \hline
0.5                  & 0.95      & 0.93   & 0.94 & 91.86\% & 0.88       & 0.47   & 0.61 & 44.90\% \\ \hline
0.6                  & 0.93      & 0.91   & 0.92 & 89.91\% & 0.85       & 0.45   & 0.59 & 41.64\% \\ \hline
0.7                  & 0.89      & 0.87   & 0.88 & 84.34\% & 0.77       & 0.41   & 0.54 & 35.92\% \\ \hline
0.8                  & 0.8       & 0.78   & 0.79 & 73.62\% & 0.68       & 0.36   & 0.47 & 30.96\% \\ \hline
0.9                  & 0.5       & 0.49   & 0.5  & 37.88\% & 0.44       & 0.23   & 0.31 & 16.83\% \\ \hline
\end{tabular}
\caption{Table Detection scores on the borderless split of the custom dataset}
\label{tab:table_detection_borderless_split}
\end{table}

% Scores for coloured table detection BUDDI vs amazon
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{IoU} & \multicolumn{4}{c|}{BUDDI Dexter}   & \multicolumn{4}{c|}{AMAZON Textract} \\ \cline{2-9} 
                     & Precision & Recall & F1  & mAP      & Precision  & Recall & F1   & mAP     \\ \hline
0.5                  & 1.0       & 1.0    & 1.0 & 100.00\% & 1.0        & 0.8    & 0.89 & 80.00\% \\ \hline
0.6                  & 1.0       & 1.0    & 1.0 & 100.00\% & 1.0        & 0.8    & 0.89 & 80.00\% \\ \hline
0.7                  & 1.0       & 1.0    & 1.0 & 100.00\% & 1.0        & 0.8    & 0.89 & 80.00\% \\ \hline
0.8                  & 1.0       & 1.0    & 1.0 & 100.00\% & 1.0        & 0.8    & 0.89 & 80.00\% \\ \hline
0.9                  & 0.8       & 0.8    & 0.8 & 73.00\%  & 1.0        & 0.8    & 0.89 & 80.00\% \\ \hline
\end{tabular}
\caption{Table Detection scores on the coloured table split of the custom dataset}
\label{tab:table_detection_coloured_table_split}
\end{table}


% Scores for partial bordered table detection BUDDI vs amazon
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{IoU} & \multicolumn{4}{c|}{BUDDI Dexter}   & \multicolumn{4}{c|}{AMAZON Textract} \\ \cline{2-9} 
                     & Precision & Recall & F1  & mAP      & Precision  & Recall & F1   & mAP     \\ \hline
0.5                  & 1.0       & 1.0    & 1.0 & 100.00\% & 1.0        & 0.5    & 0.67 & 50.00\% \\ \hline
0.6                  & 1.0       & 1.0    & 1.0 & 100.00\% & 1.0        & 0.5    & 0.67 & 50.00\% \\ \hline
0.7                  & 0.9       & 0.9    & 0.9 & 87.00\%  & 0.8        & 0.4    & 0.53 & 38.00\% \\ \hline
0.8                  & 0.8       & 0.8    & 0.8 & 76.00\%  & 0.8        & 0.4    & 0.53 & 38.00\% \\ \hline
0.9                  & 0.5       & 0.5    & 0.5 & 35.00\%  & 0.8        & 0.4    & 0.53 & 38.00\% \\ \hline
\end{tabular}
\caption{Table Detection scores on the partial bordered table split of the custom dataset}
\label{tab:table_detection_partial_bordered_table_split}
\end{table}


% ABLATION STUDY FOR CELL DETECTION

% Scores for bordered cell detection BUDDI vs amazon
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{IoU} & \multicolumn{4}{c|}{BUDDI Dexter}   & \multicolumn{4}{c|}{AMAZON Textract} \\ \cline{2-9} 
                     & Precision & Recall & F1   & mAP     & Precision  & Recall & F1   & mAP     \\ \hline
0.5                  & 0.98      & 0.98   & 0.98 & 96.97\% & 0.92       & 0.98   & 0.95 & 94.92\% \\ \hline
0.6                  & 0.98      & 0.98   & 0.98 & 96.39\% & 0.91       & 0.96   & 0.93 & 92.82\% \\ \hline
0.7                  & 0.98      & 0.98   & 0.98 & 95.96\% & 0.88       & 0.94   & 0.91 & 88.13\% \\ \hline
0.8                  & 0.97      & 0.97   & 0.97 & 95.25\% & 0.56       & 0.6    & 0.58 & 35.79\% \\ \hline
0.9                  & 0.97      & 0.97   & 0.97 & 95.11\% & 0.07       & 0.08   & 0.07 & 0.75\%  \\ \hline
\end{tabular}
\caption{Cell Detection scores on the bordered table split of the custom dataset}
\label{tab:cell_detection_bordered_table_split}
\end{table}


% Scores for borderless cell detection BUDDI vs amazon
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{IoU} & \multicolumn{4}{c|}{BUDDI Dexter}   & \multicolumn{4}{c|}{AMAZON Textract} \\ \cline{2-9} 
                     & Precision & Recall & F1   & mAP     & Precision  & Recall & F1   & mAP     \\ \hline
0.5                  & 0.88      & 0.76   & 0.82 & 67.11\% & 0.37       & 0.39   & 0.38 & 16.08\% \\ \hline
0.6                  & 0.84      & 0.72   & 0.77 & 60.35\% & 0.24       & 0.25   & 0.24 & 7.21\%  \\ \hline
0.7                  & 0.79      & 0.67   & 0.73 & 53.41\% & 0.14       & 0.15   & 0.15 & 2.66\%  \\ \hline
0.8                  & 0.73      & 0.63   & 0.67 & 46.36\% & 0.06       & 0.06   & 0.06 & 0.59\%  \\ \hline
0.9                  & 0.67      & 0.58   & 0.62 & 39.93\% & 0.01       & 0.01   & 0.01 & 0.01\%  \\ \hline
\end{tabular}
\caption{Cell Detection scores on the borderless table split of the custom dataset}
\label{tab:cell_detection_borderless_table_split}
\end{table}


% Scores for coloured cell detection BUDDI vs amazon
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{IoU} & \multicolumn{4}{c|}{BUDDI Dexter}   & \multicolumn{4}{c|}{AMAZON Textract} \\ \cline{2-9} 
                     & Precision & Recall & F1   & mAP     & Precision  & Recall & F1   & mAP     \\ \hline
0.5                  & 0.98      & 0.95   & 0.96 & 92.52\% & 0.55       & 0.33   & 0.42 & 21.73\% \\ \hline
0.6                  & 0.97      & 0.94   & 0.95 & 90.43\% & 0.43       & 0.26   & 0.32 & 12.54\% \\ \hline
0.7                  & 0.97      & 0.94   & 0.95 & 90.43\% & 0.18       & 0.11   & 0.13 & 1.92\%  \\ \hline
0.8                  & 0.94      & 0.91   & 0.93 & 86.32\% & 0.02       & 0.01   & 0.01 & 0.02\%  \\ \hline
0.9                  & 0.91      & 0.88   & 0.9  & 80.33\% & 0          & 0      & 0    & 0.00\%  \\ \hline
\end{tabular}
\caption{Cell Detection scores on the coloured table split of the custom dataset}
\label{tab:cell_detection_coloured_table_split}
\end{table}

% Scores for partial bordered cell detection BUDDI vs amazon
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{IoU} & \multicolumn{4}{c|}{BUDDI Dexter}   & \multicolumn{4}{c|}{AMAZON Textract} \\ \cline{2-9} 
                     & Precision & Recall & F1   & mAP     & Precision  & Recall & F1   & mAP     \\ \hline
0.5                  & 1.0       & 0.94   & 0.97 & 93.94\% & 0.44       & 0.36   & 0.4  & 24.24\% \\ \hline
0.6                  & 1.0       & 0.94   & 0.97 & 93.94\% & 0.3        & 0.24   & 0.27 & 11.11\% \\ \hline
0.7                  & 0.97      & 0.91   & 0.94 & 89.05\% & 0.22       & 0.18   & 0.2  & 8.32\%  \\ \hline
0.8                  & 0.94      & 0.88   & 0.91 & 84.36\% & 0.19       & 0.15   & 0.17 & 6.89\%  \\ \hline
0.9                  & 0.94      & 0.88   & 0.91 & 84.36\% & 0.04       & 0.03   & 0.03 & 0.38\%  \\ \hline
\end{tabular}
\caption{Cell Detection scores on the partial bordered table split of the custom dataset}
\label{tab: cell_detection_partialbordered_table_split}
\end{table}
